KBLAS: An Optimized Library for Dense Matrix-Vector Multiplication on GPU Accelerators

KBLAS is a new open source high performance library that provides optimized kernels for a subset of Level 2 BLAS functionalities on CUDA-enabled GPUs. Since performance of dense matrix-vector multiplication is hindered by the overhead of memory accesses, a double-buffering optimization technique is employed to overlap data motion with computation. After identifying a proper set of tuning parameters, KBLAS is able to efficiently run on various GPU architectures across different generations, avoiding the time-consuming step of code rewriting, while still being compliant with the standard BLAS API. Another advanced optimization technique allows to ensure coalesced memory access when dealing with submatrices, especially in the context of high level dense linear algebra algorithms. All four precisions KBLAS kernels have been leveraged to multi-GPUs environment, which requires the introduction of new APIs to ease users' experiences on these challenging systems. The KBLAS performance outperforms existing state-of-the-art implementations on all matrix sizes, achieves asymptotically up to 50% and 60% speedup on single GPU and multi-GPUs systems, respectively, and validates our performance model. A subset of KBLAS high performance kernels has been integrated into NVIDIA's standard BLAS implementation (cuBLAS) for larger dissemination, starting version 6.0.

==> Makefile <==
# LaTeX -*-Makefile-*-
#
# $HEADER$
# 

# MAIN_TEX: In order to build your document, fill in the MAIN_TEX
# macro with the name of your main .tex file -- the one that you
# invoke LaTeX on.

MAIN_TEX	= kblas.tex

# OTHER_SRC_FILES: Put in the names of all the other .tex files that
# this document depends on in the OTHER_SRC_FILES macro.  This is
# ensure that whenever one of the "other" files changes, "make" will
# rebuild your paper.

OTHER_SRC_FILES	= intro.tex summary.tex \
                  abstract.tex perf.tex rw.tex \
		  app.tex impl.tex ack.tex gpu.tex model.tex \
		  routines.tex layout.tex \
		  contrib.tex structure.tex



# BibTeX sources.  The bibliography will automatically be re-generated
# if these files change.

BIBTEX_SOURCES = kblas.bib

# xfig figures.  Will be converted to .eps and .pdf as necessary.

FIG_FILES	=

# Files that alredy exist as .png.  Will be converted to .eps and .pdf
# as necessary.

PNG_FILES	= 

# Files that alredy exist as .eps.  Will be converted to .pdf as
# necessary.

EPS_FILES	= 


# Required commands and options

LATEX		= latex
PDFLATEX	= pdflatex
DVIPS		= dvips
MAKEINDEX	= makeindex
BIBTEX		= bibtex
FIG2DEV		= fig2dev
PNGTOPNM	= pngtopnm
PNMTOPS		= pnmtops
EPS2PDF		= epstopdf
PS2PDF          = ps2pdf
PS2PDF_OPTIONS  = -sPaperSize=letter -dAutoFilterGrayImages=false \
		-dGrayDownSample=false -sGrayImageFilter=LZWEncode \
		-dAutoFilterColorImages=false -sColorImageFilter=LZWEncode \
		-dColorDownSample=false -dEmbedAllFonts=true \
		-dSubsetFonts=true
DISTILL         = distill
DISTILL_OPTIONS = -v -pagesize 612 792 pts -encodegray on -graycompr lzw \
		-graydownsample off -grayacs off -graydepth 8 \
		-subsetfonts on -embedallfonts on -pairs
PSNUP           = psnup

#########################################################################
#
# You should not need to edit below this line
#
#########################################################################

.SUFFIXES:	.tex .dvi .ps .pdf .fig .eps .png

MAIN_DVI	= $(MAIN_TEX:.tex=.dvi)
MAIN_PS		= $(MAIN_TEX:.tex=.ps)
MAIN_PDF	= $(MAIN_TEX:.tex=.pdf)
MAIN_BBL	= $(MAIN_TEX:.tex=.bbl)
MAIN_BASENAME	= $(MAIN_TEX:.tex=)
EPS_PNG_FILES	= $(PNG_FILES:.png=.eps)
EPS_FIG_FILES	= $(FIG_FILES:.fig=.eps)
PDF_FIG_FILES	= $(FIG_FILES:.fig=.pdf)
PDF_EPS_FILES	= $(EPS_FILES:.eps=.pdf)

#
# Some common target names
# Note that the default target is "ps"
#

pdf: $(MAIN_PDF)
ps: $(MAIN_PS) 

#
# Make the dependencies so that things build when they need to
#

$(MAIN_PS): $(MAIN_DVI)
$(MAIN_DVI): $(MAIN_TEX) $(CITE_TEX) $(OTHER_SRC_FILES) $(EPS_FIG_FILES) $(EPS_FILES) $(MAIN_BBL)
$(MAIN_PDF): $(MAIN_TEX) $(CITE_TEX) $(OTHER_SRC_FILES) $(PDF_FIG_FILES) $(PNG_FILES) $(MAIN_BBL) $(PDF_EPS_FILES)

#
# Search strings
#

REFERENCES = "(There were undefined references|Rerun to get (cross-references|the bars) right|No file *[aux|toc|lof|lot])"
NEEDINDEX = "Writing index file"
RERUNBIB = "No file.*\.bbl|LaTeX Warning: Citation|LaTeX Warning: Label\(s\) may"

#
# General rules
#

.fig.eps:
	$(FIG2DEV) -L eps $< $@

.fig.pdf:
	$(FIG2DEV) -L pdf $< $@

.eps.pdf:
	@if ( `which $(DISTILL) > /dev/null 2>&1` ); then \
		cmd="$(DISTILL) $(DISTILL_OPTIONS) $*.eps $*.pdf" ; \
                echo $$cmd ; \
                eval $$cmd ;\
	elif ( which $(EPS2PDF) > /dev/null 2>&1 ); then \
		cmd="$(EPS2PDF) $(EPS2PDF_OPTIONS) $*.eps " ; \
                echo $$cmd ; \
                eval $$cmd ;\
	elif ( which $(PS2PDF) > /dev/null 2>&1 ); then \
		cmd="$(PS2PDF) $(PS2PDF_OPTIONS) $*.eps $*.pdf" ; \
                echo $$cmd ; \
                eval $$cmd ;\
	else \
		echo "Cannot find ps to pdf converter :-("; \
	fi

.png.eps:
	$(PNGTOPNM) $< | $(PNMTOPS) -noturn > $*.eps

# Only run bibtex if latex has already been run (i.e., if there is
# already a .aux file).  If .aux file does not exist, then bibtex will
# be run during the .tex.dvi / .tex.pdf rules.  We don't run latex
# here to generate the .aux file because a) we don't know whether to
# run latex or pdflatex, and b) the dependencies are wrong for
# pdflatex because we may need to generate some pdf images first.

$(MAIN_BBL): $(BIBTEX_SOURCES)
	@if (test -f $(MAIN_BASENAME).aux); then \
		echo "### Running BibTex"; \
		$(BIBTEX) $(MAIN_BASENAME); \
	fi

# Macro to handle when running "latex" fails -- ensure to kill the
# .aux and .dvi files so that the next time we run "make", the
# .tex.dvi rule fires, not the .bbl or .dvi.ps rule.

DVI_FAIL = ($(RM) $(MAIN_BASENAME).aux $(MAIN_BASENAME).dvi && false)

# Main workhorse for .tex -> .dvi.  Run latex, makeindex, and bibtex
# as necessary.

.tex.dvi:
	@echo "### Running LaTeX (1)"
	$(LATEX) $* || $(DVI_FAIL)
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (2)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(NEEDINDEX) $*.log >/dev/null); then \
		echo "### Running makeindex to generate index"; \
		$(MAKEINDEX) $*; \
		echo "### Running LaTeX after generating index"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(RERUNBIB) $*.log >/dev/null); then \
		echo "### Running BibTex because references changed"; \
		$(BIBTEX) $(MAIN_BASENAME); \
		echo "### Running LaTeX after generating bibtex"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (3)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running LaTeX to fix references (4)"; \
		($(LATEX) $*) || $(DVI_FAIL); \
	fi

.dvi.ps:
	$(DVIPS) -o $*.ps $*

# Macro to handle when running "latex" fails -- ensure to kill the
# .aux file so that the next time we run "make", the .tex.pdf rule
# fires, not the .bbl rule.

PDF_FAIL = ($(RM) $(MAIN_BASENAME).aux && false)

# Main workhorse for .tex -> .pdf.  Run latex, makeindex, and bibtex
# as necessary.  Essentially the same as .tex.dvi, except
# s/latex/pdflatex/ig.

.tex.pdf:
	@echo "### Running pdfLaTeX (1)"
	$(PDFLATEX) $* || $(PDF_FAIL)
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (2)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(NEEDINDEX) $*.log >/dev/null); then \
		echo "### Running makeindex to generate index"; \
		$(MAKEINDEX) $*; \
		echo "### Running pdfLaTeX after generating index"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(RERUNBIB) $*.log >/dev/null); then \
		echo "### Running BibTex because references changed"; \
		$(BIBTEX) $(MAIN_BASENAME); \
		echo "### Running pdfLaTeX after generating bibtex"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (3)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi
	@if (egrep $(REFERENCES) $*.log > /dev/null); then \
		echo "### Running pdfLaTeX to fix references (4)"; \
		($(PDFLATEX) $*) || $(PDF_FAIL); \
	fi

#
# graphs
#

Graph: graphs
graph: graphs
graphs:
	(cd results/la-myri; ./geplot)

#
# Just for fun
#

RUN_PSNUP = $(PSNUP) -d -b2 -m10 -pletter
1: $(MAIN_PS)
	num_pages="`psnup -1 $(MAIN_PS) bogus.ps 2>&1 | grep Wrote | cut -dW -f2- | awk '{ print $$2 }'`"; \
	$(RM) bogus.ps; \
	$(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi; \
	if test "$$?" != "0"; then \
	  num_pages="`expr $$num_pages + 1`"; \
	  $(RUN_PSNUP) -$$num_pages $(MAIN_PS) one-page.ps; \
	fi
	$(RUN_PS2PDF) one-page.ps
	$(RM) one-page.ps

#
# Standard targets
#

clean:
	$(RM) *~ *.bak *%
	$(RM) *.log *.aux *.dvi *.blg *.toc *.bbl *.lof *.lot \
		*.idx *.ilg *.int *.out */*.aux \
		$(EPS_PNG_FILES) $(EPS_FIG_FILES) $(PDF_FIG_FILES) \
		 $(PDF_EPS_FILES)

distclean: clean
	$(RM) $(MAIN_PS) $(MAIN_DVI) $(MAIN_PDF)

